High-order gas-kinetic scheme with TENO class reconstruction for the Euler and Navier-Stokes equations

The high-order gas-kinetic scheme(HGKS) with WENO spatial reconstruction method has been extensively validated through many numerical experiments, demonstrating its superior accuracy efficiency, and robustness. Compared with WENO class schemes, TENO class schemes exhibit significantly improved robustness, low numerical dissipation and sharp discontinuity capturing. In this paper, two kinds of fifth-order HGKS with TENO class schemes are designed. One involves replacing WENO5 scheme with the TENO5 scheme in the conventional WENO5-GKS. WENO and TENO schemes only provide the non-equilibrium state values at the cell interface. The slopes of the non-equilibrium state along with the equilibrium values and slopes, are obtained by additional linear reconstruction. Another kind of TENO5-D GKS is similar to WENO5-AO GKS. Following a strong scale-separation procedure, a tailored novel ENO-like stencil selection strategy is proposed such that the high-order accuracy is restored in smooth regions by selecting the candidate reconstruction on the large stencil while the ENO property is enforced near discontinuities by adopting the candidate reconstruction from smooth small stencils. The such TENO schemes are TENO-AA and TENO-D scheme. The HGKS scheme based on WENO-AO or TENO-D reconstruction take advantage of the large stencil to provide point values and slopes of the non-equilibrium state. By dynamically merging the reconstructed non-equilibrium slopes, extra reconstruction of the equilibrium state at the beginning of each time step can be avoided. The simplified schemes have better robustness and efficiency than the conventional WENO5-GKS or TENO5-GKS. TENO-D GKS is also as easy to develop as WENO-AO GKS to high-order finite volume method for unstructured mesh.

==> texTEST/texTEST/main.tex <==
\usepackage{epstopdf}
\begin{figure}
Blast1.eps
